High frequency trading and asymptotics for small risk aversion in a Markov renewal model

We study a an optimal high frequency trading problem within a market microstructure model designed to be a good compromise between accuracy and tractability. The stock price is driven by a Markov Renewal Process (MRP), while market orders arrive in the limit order book via a point process correlated with the stock price itself. In this framework, we can reproduce the adverse selection risk, appearing in two different forms: the usual one due to big market orders impacting the stock price and penalizing the agent, and the weak one due to small market orders and reducing the probability of a profitable execution. We solve the market making problem by stochastic control techniques in this semi-Markov model. In the no risk-aversion case, we provide explicit formula for the optimal controls and characterize the value function as a simple linear PDE. In the general case, we derive the optimal controls and the value function in terms of the previous result, and illustrate how the risk aversion influences the trader strategy and her expected gain. Finally, by using a perturbation method, approximate optimal controls for small risk aversions are explicitly computed in terms of two simple PDE's, reducing drastically the computational cost and enlightening the financial interpretation of the results.

==> input_asymptotic_proof.tex <==
\def\test{\mathbf{g}}

\begin{proof}(of Theorem \ref{thm::asymptotic}) Let us define the function $\test$ by $\eta \test := \Risk$, satisfying (look at (\ref{hjb_riskaversion}))
%
\begin{eqnarray*}
\eta\left(\mpartialts{\test}\right) - \sum_{\sym \in \pm} \min_{\ell \in \{0,1\}}  \left[  \eta \apply{\mathcal R_\sym[\ell]}{\test}  + \maxx{\barrierand\sym} - \ell \barrierand\sym \right]  & = & 0, \\
\test(T,) &=&  q^2,
\end{eqnarray*}
where $\mathcal R_\pm$ admits an affine decomposition $\mathcal{R}_{\pm}[\ell] = \mathcal{R}_{\pm}^{0} + \ell \mathcal{R}_{\pm}^{1}$, where
\begin{eqnarray}
\apply{\mathcal R_\pm^0}{\test} & := & \jumpintensitypm  \Delta \test(t,\pm q, 0), \nn \\
\apply{\mathcal R_\pm^1}{\test}  & := & \jumpintensitypm \round{\test(t,\pm q - L, 0) - \test(t,\pm q, 0)}  + \tradeintensitypm \int \Delta \test(t, q \mp k,s) \vartheta_{\pm}(dk, L). \nn
\end{eqnarray}
%
We can rearrange the operator in the PDE for $\test$ as
%
\begin{eqnarray*}
\eta\left(\mpartialts{\test}\right) -  \eta \sum_{\sym \in \pm} \apply{\mathcal R_\sym^0}{\test} - \sum_{\sym \in \pm} \min_{\ell \in \{0,1\}}  \ell   \left(\eta \apply{\mathcal R_\sym^1}{\test} - \barrierand\sym\right) + \maxx{\barrierand\sym}  & = &  \\
\eta\left(\mpartialts{\test}\right) -  \eta \sum_{\sym \in \pm} \apply{\mathcal R_\sym^0}{\test} + \sum_{\sym \in \pm}  \max_{\ell \in \{0,1\}}   \ell   \left(\barrierand\sym - \eta \apply{\mathcal R_\sym^1}{\test}\right) - \maxx{\barrierand\sym}  & = &  \\
\eta\left(\mpartialts{\test}\right) -  \eta  \sum_{\sym \in \pm} \apply{\mathcal R_\sym^0}{\test} + \sum_{\sym \in \pm}  \maxx{\barrierand\sym - \eta \apply{\mathcal R_\sym^1}{\test}} - \maxx{\barrierand\sym}.  \\
\end{eqnarray*}
%
Using the development 
%
\begin{eqnarray*}
\maxx{x-\varepsilon} = \maxx{x} - \varepsilon \indicator{x>0} + z(x),
\end{eqnarray*}
%
where $z(x)$ is a non-negative $o(\eta)$ for $\eta\rightarrow 0$ satifying
%
\begin{eqnarray*}
\vert z(x) \vert \leq \vert \epsilon \vert \indicator{\vert x \vert < \vert \epsilon \vert},
\end{eqnarray*}
%
we can write the PDE for $\test$ as
%
\begin{eqnarray*}
\apply{\mathcal A}{\test} + Z^{(\eta)}(t,s,q) := \mpartialts{\test} -  \sum_{\sym \in \pm} \apply{\mathcal R_\sym^0}{\test} - \sum_{\sym \in \pm}  \apply{\mathcal R_\sym^1}{\test}\indicator{\barrierand\sym > 0} + Z^{(\eta)}(t,s,q) & = & 0, \\
\test(T,) &=&  q^2,
\end{eqnarray*}
%
where 
\begin{eqnarray*}
Z^{(\eta)}t,s,q) & := & \frac{1}{\eta} \sumpm \maxx{G_\sym(t,s) - \eta \apply{\mathcal R_\sym^1}{\test}}-\maxx{G_\sym(t,s)} \geq 0, \\
\abs{Z^{(\eta)}t,s,q)} &\leq & \sumpm \abs{\apply{\mathcal R_\sym^1}{\test}} \indicator{\abs{G_\sym(t,s)} < \eta \abs{\apply{\mathcal R_\sym^1}{\test}}} =:  \overline Z^{(\eta)}(t,s,q).
\end{eqnarray*}
%
We claim that we can approximate $\test$ by the solution of 
%
\begin{eqnarray*}
\apply{\mathcal{A}}{\tilde\test} = 0 \for \tilde\test(T,)  = q^2,
\end{eqnarray*}
%
for which we are able to find a semi-explicit solution. Using the ansatz
%
\begin{eqnarray*}
\tilde \test(t, s, q) & := & q^2 + 2 q  \zeta_1(t,s) + \zeta_0(t,s),
\end{eqnarray*}
%
and injecting in the previous PDE, we obtain \marginpar{calculation are commented}
\begin{align*}
\apply{\mathcal R_\pm^0}{\test} 
%&= \jumpintensitypm \round{ ( \pm q )^2-  q ^2 + (\pm q ) \zeta_1(t,0) - q \zeta_1(t, s) + \Delta\zeta_0(t,0)}   \\
& =  \jumpintensitypm \round{ 2q  \round{\pm \zeta_1(t,0) - \zeta_1(t, s)} + \Delta  \zeta_0(t,0)},    \\
\apply{\mathcal R_\pm^1}{\test}
%&= \jumpintensitypm \round{(\pm q -  L)^2 - (\pm q )^2 +  (\pm q  -  L)\zeta_1(t,0) - (\pm q ) \zeta_1(t,0)}  \\
%& +  \tradeintensitypm \int \round{ (q - \pm k)^2-q^2 + (q - \pm k)\zeta_1(t, s)-q \zeta_1(t, s)}  \vartheta_{\pm}(dk,L)  \\
%&= \jumpintensitypm \round{ L^2 \mp2  L q  - \zeta_1(t,0)} +  \tradeintensitypm \int \round{k^2 \mp2 q k  \mp k \zeta_1(t, s)}  \vartheta_{\pm}(dk,L), \\
%&= \jumpintensitypm \round{ L^2 \mp2  L q  - \zeta_1(t,0)} +  \tradeintensitypm \round{ \Phi^2_\pm( L) \mp2q  \Phi^1_\pm( L) \mp \Phi^1_\pm( L) \zeta_1(t, s)}  \\
& = \mp 2q \round{\jumpintensitypm +  \tradeintensitypm \Phi^1_\pm( L)}   +  {\jumpintensitypm \round{ L^2 -  2L  \zeta_1(t,0)} +  \tradeintensitypm\round{ \Phi^2_\pm( L) \mp 2 \Phi^1_\pm( L) \zeta_1(t, s)}}.
\end{align*}
%
Splitting by the degree in $q$, and dividing by $2$, we have
\begin{eqnarray*}
\mpartialts{ \zeta_1} - 
\underbrace{\sumpm h_\sym(s) \round{\sym \zeta_1(t,0) - \zeta_1(t, s)}}_{= \drift \zeta_1(t,0) - \vol \zeta_1(t,s)} +  
\sumpm \sym  \round{h_\sym(s) +  \lambda_\sym(s) \Phi^1_\sym(L)} \underbrace{\indicator{\barrierand\sym > 0}}_{= \hat{\ell}_\pm(t,s)}  &=& 0,\\
\zeta_1(T,) &= & 0,
\end{eqnarray*}
which is the PDE characterization of $\risk_1$ (\ref{eqzeta1}), while the probabilistic representation of $\risk_1$ at (\ref{eq::zeta1_proba}) derives immediately from Proposition \ref{prop::zeta1}. Grouping the remaining terms non multiplying $q$, we obtain the characterization (\ref{eqzeta0}). 

%We recall that, by the previous argument, $\tilde\test \geq \test \geq 0$, which is a $\eta$-uniform bounds for $\Risk$.
%
We now prove that $\delta := \tilde\test - \test \downarrow 0$, for $\eta \downarrow 0^+$, which would prove that we have provided an $o(\eta)$-approximation of the exact solution $\Risk$ (i.e. that $R^{(\eta)}$ in the theorem is $o(\eta)$): since $\mathcal A$ is linear, $\delta$ solves
%
\begin{eqnarray}
\apply{\mathcal A}{\delta} - Z^{(\eta)}(t,s,q) = 0 \for \delta(T,)=0.
\end{eqnarray}
%
We can write $\mathcal A$ as 
\begin{eqnarray*}
\apply{\mathcal A}{\delta} 
&:=& \mpartialts{\delta} -  \sum_{\sym \in \pm} \apply{\mathcal R_\sym^0}{\delta} - \sum_{\sym \in \pm}  \apply{\mathcal R_\sym^1}{\delta} \underbrace{\indicator{\barrierand\sym > 0}}_{\hat\ell_\sym(t,s)}.
\end{eqnarray*}
Now,  the infinitesimal generator of the Markov process $(t, S_t, Q_t)$ under the trading strategy $\hat{\bf{\bell}}$ is given exactly by
\begin{eqnarray*}
\mpartialts \varphi 
- \sum_{\sym\in\pm} { \jumpintensityand{\sym} \Delta \varphi\round{t, 0, \sym q- \hat\ell_\sym(t,s) L} + \tradeintensityand{\sym} \int \Delta \varphi\round{t, s, q - \sym k\hat\ell_\sym(t,s)} \vartheta_\sym(dk,L)}, 
% \\ = \mpartialts{\delta} -  \sum_{\sym \in \pm} \apply{\mathcal R_\sym\left[\hat\ell\right]}{\delta} &=&  
\end{eqnarray*}
i.e. $\apply{\mathcal A}{\varphi}$. This induces the probabilistic representation
%
\begin{eqnarray*}
\delta(t,s,q) &= \mathbb E_{t,s,q}\left[ \int_t^T \overline Z^{(\eta)}(t, S_u, Q_u) du \right] \downarrow 0 \for \eta \downarrow 0^+
\end{eqnarray*}
%
by the Monotone Convergence Theorem. Moreover, since $Z^{(\eta)}\geq 0$, by the same probabilistic argument, we prove that $R^{(\eta)} \geq 0$.
\marginpar{stability principle instead otherwise?}
\end{proof}

==> input_proposition_zeta1.tex <==


Before proving the theorem, we need an auxiliary result characterizing the expectation of the terminal inventory under a particular class of Markov strategy.


\begin{Proposition}\label{prop::zeta1}
Under a given Markov strategy ${\bf\bell} :=\round{\ell_{\pm}(t,s)}$,
%
\begin{eqnarray*}
\E_{t, s, i, y}\left[ Y_{T}\following{{\bf\bell}}\right] = y + i g(t,s),
\end{eqnarray*}
%
where $g$ is the viscosity solution of 
%
\begin{eqnarray} \label{eq::strategy}
\mpartialts{g} & & 
\\ -  \drift g(t,0) + \vol g(t,s) + \sumpm \sym  \round{h_\sym(s) L + \lambda_\sym(s) \Phi^1_\pm(L)} \ell_{\sym}(t, s) & = & 0 ,  \nn \\
g(T,) & = & 0 \nn
\end{eqnarray}
%
\end{Proposition}

% proof
\begin{proof}
We define $ G(t, s, i, y) := \E_{t, s, i, y}\left[Y_{T}\following{{\bf\bell}}\right]$,  which is associated to the Feymann-Kac equation
\begin{eqnarray*}
\mpartialts{G} & & \\
- \sumpm h_\sym(s) \Delta G(t, 0, \sym i, y - \sym i  L \ell_{\sym}(t,s)) - \sumpm \lambda_\sym(s) \int \Delta G(t, s, i, y - \sym i  k \ell_{\sym}(t,s)) \vartheta_{\sym}(dk, L) & = 0 ,\\
G(T,) & = \y.
\end{eqnarray*}
Using the ansatz $G(t, s, i, y) := y + i g(t,s)$, after tedious but straightforward calculations, the previous PDE becomes
\begin{eqnarray*}
i \round{\mpartialts{g}} - \sumpm h_\sym(s) \round{- \sym i  L \ell_{\sym}(t,s) + i \round{\sym g(t,0) - g(t,s)}} + \lambda_\sym(s) \round{- \sym i  \Phi^{1}_{\pm}(L) \ell_{\sym}(t,s)} & =  & 0 ,\\
g(T,) & = & 0,
\end{eqnarray*}
%
which is, dividing by $i$ and rearranging the terms, equivalent to (\ref{eq::strategy}).
\end{proof}


==> input_theta_probabilistic_representation.tex <==
\newcommand{\lawequiv}[1]{\left\{ #1\right\}}
\subsection{The probabilistic representation}

We now investigate further bounds for $\theta(t,s)$, as well as its asymptotic behavior for large horizons, using a probabilistic approach based on the representation (\ref{thetaproba}).
\pietro{}{The probabilistic angle allows to exploit the Markov property of the stock price to capture information that are hidden in the probabilistic representation of Lemma \ref{lemma::theta}.}In order to emphasize the dependence on the horizon $T$, we write $\thetaT(t,s)$ for $\theta(t,s)$ and define the conditional mean of the next jump w.r.t. to the elapsed time as
\begin{eqnarray}\labeleq{def_tilde_alpha}
\tilde\alpha(s) &:=& \condprob{E}{}{J_1\condto \blue{I}_{0} =+ 1,S_0 = s } \for s\in\Rplus,
\end{eqnarray}
Notice that, by its very definition,
\begin{eqnarray}
\tilde\alpha(s) &:=& \condprob{E}{}{J_1\condto T_1\geq s, J_{0} =+1 } =\condprob{P}{}{B_1\condto T_1\geq s, J_{0} =+ 1}  \for s\in\Rplus\nn ,
\end{eqnarray}
where $B_1$ is given in \refequation{Bn}.
%\end{Definition}
\begin{Lemma}\label{lemmaBayes}
For a Markov Renewal Process $(J_k,T_k)$ on a finite state space $E$ with 
\begin{eqnarray*}
Q_{ij} := \condprob{P}{}{J_k=j \vert J_{k-1}=i} \for F_{ij} := \condprob{P}{}{T_k-T_{k-1} \leq s \vert J_k=j, J_{k-1}=i}\for i,j\in E , 
\end{eqnarray*}
we have
\begin{eqnarray}
\condprob{P}{}{J_k = j \vert J_{k-1} = i , T_k-T_{k-1} \geq s} = Q_{ij} \frac{1-F_{ij}(s)}{1- \sum_{j\in E} Q_{ij} F_{ij}(s)} , \;\;\;i,j\in E . \labeleq{_alphatilde}
\end{eqnarray}
\end{Lemma}
%%
\begin{proof}
A simple Bayes argument gives
\begin{eqnarray*}
&&\condprob{P}{}{J_k = j \vert J_{k-1} = i , T_k-T_{k-1} \geq s} =  \frac{\condprob{P}{}{J_k = j , T_k-T_{k-1} \geq s \vert J_{k-1} = i}}{\condprob{P}{}{T_k-T_{k-1} \geq s \vert J_{k-1} = i}}  \\
&=& \frac{\condprob{P}{}{T_k-T_{k-1} \geq s \vert J_{k-1} = i , J_k = j } \condprob{P}{}{J_k=j\vert J_{k-1}=i}}{\sum_{j\in E} \condprob{P}{}{T_k-T_{k-1} \geq s \vert J_{k-1} = i , J_k = j}\condprob{P}{}{J_k=j\vert J_{k-1}=i}} \\
&=& \frac{Q_{ij}\left(1-F_{ij}(s)\right)}{\sum_{j\in E} Q_{ij}\left(1-F_{ij}(s)\right)} =  Q_{ij} \frac{1-F_{ij}(s)}{1- \sum_{j\in E} Q_{ij} F_{ij}(s)} .
\end{eqnarray*}
\end{proof}
\begin{Corollary}\label{cor::tilde_alpha} 
For $s\in\Rplus$,
\begin{eqnarray*}
\tilde\alpha(s) &=& \sum_{\sym\in\pm} \sym\left(\frac{1+\sym\alpha}{2}\right)\left(\frac{1-F_{\sym}(s)}{1- F(s)}\right). 
\end{eqnarray*}
In particular i) $\tilde{\alpha}(0)=\alpha$, while ii) if marks and tick times are independent, $\tilde\alpha(s)$ $\equiv$ $\alpha$.
\end{Corollary}
\begin{proof}
The claimed expression  for $\tilde\alpha(s)$ follows from Lemma \ref{lemmaBayes} applied to the MRP driving the stock price: indeed, using the notation of the lemma with
$$
E = \pmset  \for  Q_{ij} = \frac{1+ij\alpha}{2} \for F_{ij} = \sum_{\sym\in\pm} F_\sym 1_{\{ij=\sym\}}, 
$$
we have for any $i$ $\in E$: 
%\marginpar{ Lien avec $\tilde\alpha^s$: $S_0$ $=$ $s$ et ici $S_k\geq$ $s$} 
$$
\sum_{j\in E} j \condprob{P}{}{J_1 = j   \vert J_{0} = i , T_1 \geq s}
= \sum_{j\in E} j  Q_{ij} \frac{1-F_{ij}(s)}{1- \sum_{j\in E} Q_{ij} F_{ij}(s)} = \sum_{\sym\in\pm} \sym\left(\frac{1+\sym\alpha}{2}\right)\left(\frac{1-F_{\sym}(s)}{1- F(s)}\right).
$$
In order to prove that $\tilde\alpha(0)$ $=$ $\alpha$, we can either show it directly from \refequation{def_tilde_alpha}, since
$$
\tilde\alpha(0) = \condprob{E}{}{J_1 \vert I_0 = +1,S_0 = 0}  = \condprob{E}{}{B_1} = \alpha,
$$
or by the analytic formula \refequation{_alphatilde}, noticing that (no masses in $0$ are assumed) 
$
F(0)=F_+(0)=F_-(0)=0.
$
For the final assertion,  one can use \refequation{_alphatilde}, noticing that if  the tick time $(N_t)$ and mark process $(J_k)$ are independent, then
$$
F_+ = F_- = F \Rightarrow \tilde\alpha(s) = \sum_{\sym\in\pm} \sym\,\frac{1+\sym\alpha}{2} = \alpha.
$$
\end{proof}

In the remaining part we describe the asymptotic behavior of $\theta$ by a standard regenerative argument.

\blue{
\begin{Proposition}\label{prop::phi_infty}
The asymptotic behaviour of $\theta^T(t,s)$ is given by
\begin{eqnarray}
\lim_{T\rightarrow\infty} \theta^T(t,s) &=& 2\delta \frac{\tilde\alpha(s)}{1-\alpha} \for \forall s\in\Rplus.
\end{eqnarray}
\end{Proposition}
\begin{proof}\marginpar{hope it is more convincing}
We assume that the first jump event, under $I_0=+$ and $S_0=s$, is described by the couple $(J_1,T_1)$. At time $T_1$ ($T_1<\infty$, since the process $N_t$ is assumed non-explosive), $P_{T_1} = 2\delta J_1$, $I_{T_1} = J_1$,  $S_{T_1} = 0$, while
\begin{align*}
\condprob{E}{}{P_{T_1} \condto P_0=0, S_0=s, I_0=+1 } &=2\delta \condprob{E}{}{J_{1} \condto S_0=s, I_0=+1 } = 2\delta \tilde\alpha(s). 
\end{align*}
We notice that $(P_u)_{u\geq T_1}$ conditionally on $(T_1,J_1)$ is given by $P_{T_1}$ plus the independent product of $J_1$ times an independent stochastic process (driven by the same dynamic of $(P_{t})$ conditionally on $S_0=P_0=0$ and $I_0=+1$), as shown by
\begin{align*}
P_t := P_{T_1} + 2\delta \sum_{k=2}^{N_t} {J_k} 
= P_{T_1} + J_1\left(2\delta  \sum_{k=2}^{N_t}\prod_{i=1}^{k} B_i\right),
\end{align*}
which proves that
\begin{align*}
\lawequiv{P_t \condto J_1,T_1} \equiv P_{T_1} + J_1 \hat P_{N_t-1} \for \hat P_{n}  \equiv 2\delta  \sum_{k=1}^{n}\prod_{i=1}^{k} B_i, 
\end{align*}
where $(\hat P_{n})$ is independent from $J_1$. Now, by tower conditioning w.r.t. to $(T_1,J_1)$,
\begin{align*}
\lim_{T\rightarrow\infty}\theta^T(t,s)  & = \lim_{t\rightarrow\infty}\theta^t(0,s) = \lim_{t\rightarrow\infty}\condprob{E}{}{P_{t} \condto P_0=0, S_0=s, I_0=+1 }  = 2\delta\tilde\alpha(s) + 2\delta\tilde\alpha(s) \lim_{n\rightarrow\infty} \mathbb E\left[\hat P_n\right] \\
& = 2\delta\tilde\alpha(s) + 2\delta\tilde\alpha(s) \sum_{k=1}^{\infty} \alpha^k =  2\delta\tilde\alpha(s) \sum_{k=0}^{\infty} \alpha^k = 2\delta\round{\frac{\tilde \alpha(s)}{1-\alpha}},
\end{align*}
which concludes the proof. Notice that key element in the proof is finding a random time where $(P_t)$ ``regenerates" (we can apply somehow the Markov property), and from which its average long-run behavior can be deduced only by the embedded Markov chain $(J_k)$ associated to the Markov renewal process $(P_t)$.
\end{proof}
}



